Tit-for-Token: Understanding Fairness when Forwarding Data by Incentivized Peers in Decentralized Storage Networks

Decentralized storage networks offer services with intriguing possibilities to reduce inequalities in an extremely centralized market. The challenge is to conceive incentives that are fair in regard to the income distribution among peers. Despite many systems using tokens to incentivize forwarding data, like Swarm, little is known about the interplay between incentives, storage-, and network-parameters. This paper aims to help fill this gap by developing Tit-for-Token (Tit4Tok), a framework to understand fairness. Tit4Tok realizes a triad of altruism (acts of kindness such as debt forgiveness), reciprocity (Tit-for-Tat's mirroring cooperation), and monetary rewards as desired in the free market. Tit4Tok sheds light on incentives across the accounting and settlement layers. We present a comprehensive exploration of different factors when incentivized peers share bandwidth in a libp2p-based network, including uneven distributions emerging when gateways provide data to users outside the network. We quantified the Income-Fairness with the Gini coefficient, using multiple model instantiations and diverse approaches for debt cancellation. We propose regular changes to the gateway neighborhood and show that our shuffling method improves the Income-Fairness from 0.66 to 0.16. We quantified the non-negligible cost of tolerating free-riding (altruism). The performance is evaluated by extensive computer simulations and using an IPFS workload to study the effects of caching.

==> tex/core3_backup.tex <==
\section{Tit-for-Token}
\label{sec:tit-for-token-model}
%The bandwidth incentive model described in~\autoref{sec:tit-for-token-model} is inspired in properties desired in decentralized storage networks, taking as a reference the Swarm network. 

This section presents our system model bridging network and economics aspects of modern p2p-based storage system with the \emph{Tit-for-Token} concept; besides, it gives preliminaries to  delve into the fairness of \emph{Tit-for-Token} and a diverse selection of payment mechanisms that are presented in the coming sections.   
\veg{This model makes no reference to the limited free service. How the chunks are counted in the pairwise balance?}

%CITE THE SURVEY ~\cite{ihle2023incentive}

\subsection{Tit-for-Token Model}
\begin{figure*}
    \centering    \includegraphics[width=0.75\textwidth]{images/SystemModel.pdf}

    \caption{\tftok{} includes  routing and accounting layers. The settlement layer transfers tokens through off-chain payments. The exchange layer is excluded. 1) A gateway requests a chunk, and 2-4) forwarding operators route the request to a storer and the chunk back to the gateway, sometimes for free or in reciprocity for services.
    5) Pairwise balances are updated, and 6) an unbalanced account is 7)rebalanced through token transfer. 
    8) Tokens are sold on the exchange layer to extract monetary rewards.
    }
    \label{fig:system_model}
\end{figure*}

We assume a layered model containing routing, accounting, settlement, and exchange layers, summarized in Figure~\ref{fig:system_model}.


We assume a distributed storage system comprised of peers $\{p_n;n\in N\}$, connected via a Kademlia DHT table.
Every peer maintains a routing table, according to the Kademlia algorithm. 
This table contains at most $k$ other peers in each bucket.
These connections are used in both directions, meaning if peer $p_1$ is part of $p_2$'s routing table, then also $p_2$ is part of $p_1$'s routing table.
We are interested to study how the tokens paid by gateways get distributed in a well-functioning network.
\gi{It is not clear why we focus on gateways. We need to introduce intution that gateways lead to decentralization early in the text, possibly together with the definition.}
We, therefore, assume that all peers are well-behaved, reply to requests and settle their debt according to a shared protocol.
We assume no significant churn, massive failures, or massive amounts of sybils exist in the system.


Peers may initialize the download of chunks. 
In this case, requests and replies including the chunk are routed through the Kademlia network using forwarding Kademlia on the routing layer.
Peers that initialize downloads by requesting a chunk are called gateways.
\gi{This is the second definition of a 'gateway', different from the first one in S.3.}
We assume that all, or at least some gateways, are willing to pay for the service of downloading a chunk through a token transfer.
A peer can reply to a request in two ways. Either it forwards the request to a different peer, and later 
forwards the chunk back to the requestor, or it retrieves the reply from local storage.
We say that in the first case, the peer performs a \textit{forwarding action}, and in the latter, it performs a \textit{storing action}.
The upload of chunks functions similar to downloads, and can use the same layers. However, since uploads are less frequent, we focus on the retrieval of chunks. Also, in Swarm, chunk uploads are part of storage incentives.

On the \textit{accounting layer}, peers maintain pairwise balances associated with each connection in the routing layer.
Pairwise balances are not verifiable to others and thus do not need transactional or enforcement mechanisms.
When receiving a chunk from a neighbor, balances are updated, and the sending neighbor is credited some accounting units.
This happens independently on every hop in the route.
%
We note that each peer $p_i$ performing a forwarding action is credited some amount $c_i^{in}$ from the previous peer on the route, and again credits some amount $c_i^{out}$ to the next peer. We say that the difference between these two amounts $c_i^{in} - c_i^{out}$ is the \textit{reward} $p_i$ receives for forwarding.
The reward for storing is simply the credited amount. We note that the reward for a storing action is incentivizing bandwidth usage. 
The incentivization of long-term storage is done through storage incentives, which are out of scope for this paper.

On the \textit{settlement layer}, peers transfer utility tokens to each other.
Settlements are used to rebalance pairwise accounts and may result in a monetary transfer.
We assume settlements are realized through an off-chain payment, similar to Swarm's signed receipts.
We also assume the existence of an exchange layer, where utility tokens received through a transfer can be converted to native currency.

We do not model the exchange layer or the detailed mechanisms of token transfers, 
but assume they ensure finality and incur no fee or added cost.
Such assumptions can be approximated by off-chain solutions where fees can be amortized over many individual settlements~\cite{offchain}.

We assume there is a fixed exchange rate from utility tokens to accounting units and assume that utility tokens have a stable market price reflecting their usefulness.
In the rest of this paper, we mostly ignore utility tokens. Instead, we say that a certain amount of accounting units is settled if the corresponding amount of utility tokens are being transferred.

\subsection{Debts: Forgiveness and Payments}

Reciprocity describes the idea that services peers provide to each other may balance out, or that service received may be paid for by providing service.
In our payment model, this implies that accounting units peers credit to each other may balance out, without requiring settlement via utility tokens.
Therefore, peers maintain a pairwise balance for connections in their routing table, which they increment or decrease with the credited accounting units 
when receiving or providing service from/to each other.
Peers provide service without requiring settlement, as long as this balance is below a given threshold.

Figure~\ref{fig:reciprocation} shows an example of reciprocity. Peers A and B initialize the pairwise accounting channel with balance zero and a threshold in step $(1)$. A sends a request and goes into debt to B, and the balance tilts towards A in step $(2)$. Then B sends a request, and A provides the service, and the balance goes back around zero in step $(3)$. In step $(4)$,
B has reached the maximum debt and hits the threshold. A stops providing service until B brings the balance below the threshold again.
\gi{Figure 3 description seems to duplicate the description in the text. Maybe figure description can be shortened to just 'Example of pairwise accounting'.}

\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{
    \input{tex/plots/reciprocity_figure.tex}}
    \caption{Example for reciprocity. Peers A and B have a pairwise accounting channel. They pay for the service by service and keep the balance below the threshold.}
    \label{fig:reciprocation}
\end{figure}


==> tex/core5_payment_models.tex <==
\section{Incentive Mechanisms}
\label{sec:payment_models}
\lj{Should that be settlement mechanism?}
In this section, we refine our Tit-for-Token model with
distance-based rewards, reciprocity, and limited free service.
We first describe how these three affect pairwise accounting.
We explain the different parameters and challenges these mechanisms pose to fairness.
%
% are realized on the accounting layer, and describe their motivation, benefits and challenges. 
\veg{The sentence above is weird (mechanisms have no motivation). I would remove it. Besides do not use mechanisms for other things that are not incentives - Then if you use the word mechanism alone it will be difficult to know what are we talking about like in the following sentence.}
%
In Section~\ref{sec:settle} we explain the effect these mechanisms have on token settlements (settlement layer).
% In Section~\ref{sec:evaluation} we evaluate the effectiveness of the mechanisms for different parameter and network settings and evaluate their effect on \incomefairness.

\subsection{How many accounting units are credited?}
\label{sec:distancerewards}
We consider two models for how many accounting units peers credit each other for replying to a request: constant reward, and distance-based reward.
This happens on the accounting layer of our model.
Remember that for forwarding actions, reward $c_i^{in} - c_i^{out}$ is the difference between accounting units credited to a peer $p_i$ and by $p_i$ to the next peer.
Here $c_i^{out}=c_{i+1}^{in}$


\textbf{Constant reward.} 
In this model, all peers on the path of a request receive the same reward.
\lj{The paragraph below is of little relevance and could be removed:}
Thus, the credited amounts between two peers are proportional to the length of the tail of the route.
This is an abstract model which does have some drawbacks in practice. 
For example, suboptimal paths, i.e., longer paths, require a larger payment from the gateway but involved peers receive the same reward. Thus, peers are not incentivized to find optimal routes.
Similarly, it is unclear how the gateway should verify the length of the route.
However, this model is useful as a baseline, as it shows how actions are distributed in the network.
\gi{We can indeed cut this paragraph to two sentenced explaining that we need this only as a baseline in evaluations. However it is not clear what is meant by 'how actions are distributed in the network', this is vague.}


\textbf{Distance-based reward.} This model uses the XOR distance to find the amount of payment. 
The payment $c_i^{in}$ is calculated based on the distance of peer $p_i$ from the chunk.
The reward received by $p_i$ for a forwarding action is therefore determined by the distance over which $p_i$ forwards the request and reply.
In this way, peers are motivated to forward to the peer with the shortest possible distance to the destination.
In this model, payments do not depend on knowledge of the path, e.g., the payment the gateway makes to the first hop in the path does not depend on the length of the path.

Distance-based rewards are in use in the Swarm network.
As the Swarm network, we use Equation~\ref{eq:maxPO} to determine $c_i^{in}$.
Here \mp is a configurable parameter explained below.
\gi{Is \mp a threshold parameter in pairwise accounting? If so it shouhld be mentioned here already.}
$\textit{CommonBitsInPrefix}$ returns the number of bits common in the prefix of two addresses. 
The constant $+1$ in the equation ensures that the last peer in the route (performing the storage action) receives at least one accounting unit.
We note that in Swarm, $c_i^{in}$ is additionally multiplied by a constant \textit{price}, which we omit for simplicity.
% The $\textit{price}$ is a constant used in Swarm which we omit for the rest of this paper.

\begin{equation}
\label{eq:maxPO}
    c_i^{in} = (\mp - \textit{CommonBitsInPrefix}(p_i, \textit{chunkAddress}) + 1)
\end{equation}
\gi{Equation needs a number in text. Is it 6.2. mentioned below?}
We could find no information in Swarm documents about how to initialize $\mp$, while oral communication gave an idea that
it should not be initialized too small.
\gi{'Should not be too small is vague', smaller than what?. I would rephrase it as: "While there is no information in Swarm documents about how to initialize $\mp$, empirically in Swarm deployment it is picked less than n.}
We initialize $\mp=\delta+\alpha$. 
Here $\delta$ is the storage depth, another parameter in Swarm, determining whether a peer is responsible to store a chunk.
A peer $p_i$ is responsible to store a chunk if $\textit{CommonBitsInPrefix}(p_i, \textit{chunkAddress})\geq \delta$.
Setting $\mp \geq \delta$ ensures that $\mp > \textit{CommonBitsInPrefix}(p_j, \textit{chunkAddress})$ holds for a peer $p_j$ not storing a chunk. 
Peer $p_j$ can forward the request to a different peer $p_{j+1}$ closer to the chunk, and receive $c_j^{in}-c_{j+1}^{in}>0$. 
Thus a forwarding peer receives a non-zero reward.
The parameter $\alpha$ is configurable. A larger $\alpha$ results in an additional reward given to the last peers in the route.
Figure~\ref{fig:maxpo_example} shows an example of how peers pay using Equation~\ref{eq:maxPO}.
\gi{No equation number in text.}

\input{tex/plots/omega_11_16_30.tex}

Using distance-based rewards, the same action, i.e., forwarding a request and response, may trigger different rewards.
\gi{Seems to be a redundant statement.}
Similarly, the amount of accounting units, a gateway has to credit to its neighbor, to receive a specific chunk, depends on the distance of the neighbor to that chunk. 
Thus a gateway connected to many peers, or an operator controlling multiple gateways can receive the same service for fewer accounting units.
\gi{The previous sentence a bit unclear and needs a rephrasing. Maybe: 'recieve same service at lower costs'?}
In Section~\ref{sec:evalmp} we analyze the suitable choices of the \mp parameter and show the effect distance-based rewards have on \incomefairness in Section~\ref{sec:fairaccounting}.
We also evaluate the effect of pooled connections from multiple gateways in Section~\ref{sec:clique}.

\subsection{Reciprocity}


%\begin{figure}
%    \centering
%    \begin{subfigure}[b]{0.24\textwidth}
%    \includegraphics[width=\textwidth]{images/recipro_1.pdf}
%    \caption{}
%    \label{subfig:reciprocation_a}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}[b]{0.24\textwidth}
%    \includegraphics[width=\textwidth]{images/recipro_2.pdf}
%    \caption{}
%    \label{subfig:reciprocation_b}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}[b]{0.24\textwidth}
%    \includegraphics[width=\textwidth]{images/recipro_3.pdf}
%    \caption{}
%    \label{subfig:reciprocation_c}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}[b]{0.24\textwidth}
%    \includegraphics[width=\textwidth]{images/recipro_4.pdf}
%    \caption{}
%    \label{subfig:reciprocation_d}
%    \end{subfigure}
%    \caption{}
%    \label{fig:}
%\end{figure}

A larger threshold parameter can increase reciprocity, allowing a peer to first receive multiple chunks, and later repay, by serving multiple requests.
\gi{'Intuitvely, a large threshold parameter.' This is intuition only at this stage, we demonstrate this only later.}
However, the a small threshold limits how many chunks a peer may have to provide to spurious neighbors, without receiving reciprocation.
\gi{'Selfish' peer here is more clear than 'spurious'. Spurious more often means illegitimate.}
We use $\mp$ as the default threshold parameter, ensuring that at least one request can be answered on every connection before hitting the threshold.
\gi{Why we use $\mp$ here? Beacuse it is used in Swarm or for other reason?}
Peers can rebalance the threshold through a token transfer, settling the debt.

We assume that peers prefer to reciprocate bandwidth, rather than to settle debt with tokens, 
since at least outside of cloud deployements and similar payment plans, bandwidth is a replenishing resource.
\gi{We need to elaborate on this assumption. E.g. 'We assume rational peers prefer to get badwidth via reciprocity mechanism rather than paying for bandwidth with tokens, as a way to minimize costs.'}
Especially gateways connected to each other will benefit from this.
\gi{Elaborate why gateways benefit more than other nodes from this behav}
We evaluate gateways forming cliques in Section~\ref{sec:clique}. We show that, while the pose a risk to decentralization, this allows different operators running gateways neiboring in the network to receive similar benefits as a single operator pooling the connections of multipe gateways, or connecting gateways externally.
\gi{The sentence above is too long and difficult to parse.}

Reciprocity allows actions the peers perform for each other to be repaid with actions rather than by settling with tokens.
\gi{This was already said in the beginning of the section.}
Additionally, reciprocity decouples token settlements from actions performed. 
We investigate the effect of reciprocity on \incomefairness in Section~\ref{sec:settlementfairness}.

\subsection{Limited free service}
\label{sec:limitedfreeservice}
%\todo{Should be shorter}
Limited free service describes a mechanism where peers receive the ability to download at a limited download rate without requiring settlement.
\gi{We need to say explicitly that this mechanism is separate from pairwise accounting, even though it is based on it. Otherwise 'free service' can be interpreted as merely an aspect of reciprocity.}
%\todo{Update this based on social fairness.}
This mechanism is important for a DSS for two reasons. Firstly, it helps to bootstrap the user base when the project is new. Secondly, it makes services inclusive and open for a wider userbase in the long-term.   %in the Swarm network to improve inclusion.
This mechanism is realized based on the pairwise balances from the reciprocity mechanism and parametrized by a time interval $\Delta$ and 
a \refreshrate measured in accounting units.
After time $\Delta$, if a peer is in debt with a different peer, it is forgiven \refreshrate many accounting units. 
As default \refreshrate, we use half of the reciprocity threshold. 
Thus, the debt between peers is forgiven after $2$ time intervals.

The introduction of a limited free service on all connections poses a significant challenge.
While on heavily used connections, the \refreshrate may only reduce the preformed settlement with a small amount, it may completely suppress settlements on scarcely used connections. 
We show in Section~\ref{sec:settlementfairness} that
a constant \refreshrate distributes the cost of limited free service unevenly on the path, 
impacting negatively on \incomefairness.
We also show that our adjusted variant ...
\lj{Include adjustable threshold.}

\subsection{When to settle debt with tokens?}
\label{sec:settle}

% \lj{TODO: 6.4 explain how settlement works and move the current content to appendix + Fig6 pointers to the 
% Free bandwidth section shall have pointers ot the figure in the appendix. pointers to the appendix (effective download rate) 
% COrrect caption for 6.a}


When reaching the limit of the reciprocity threshold, peers need to decide to either wait for $\Delta$ time and rely on the free service or to settle debt by transferring tokens.
%
We assume that all peers make use of reciprocity and do not settle debt unless it is required. 
Peers, therefore, try to request chunks from a neighbor, from which the pairwise balance allows retrieval without a settlement. This may result in the use of suboptimal routes.
\gi{What are suboptimal routes, and why is this bad? High costs of retrival, fairness?}
We also assume that peers transfer as few tokens as possible.
\gi{Unclear, do we assume that 'peers pay as little as possible for bandwidth'?}
Thus, when requesting a chunk without free bandwidth available, a peer will only settle enough debt to be able to request the current chunk. 
We discuss different approaches to settlement in Appendix~\ref{app:paymentmodels}.

Our settlement model differs from the default settings in Swarm. According to these default settings, Gateways always settle their debt, while forwarding peers never do so.
\gi{Why 'Gateway' is capitalized here? Should it be capitalized everywhere?}
If forwarding peers never transfer tokens, Gateways may be unable to retrieve a chunk if the Gateways neighbor has reached the reciprocity threshold with its connections. We call this situation a \textit{threshold rejection}.
If forwarding peers settle debt with their neighbors, it allows them to serve more requests and receive income based on the forwarded distance.
\gi{We explain default settings in Swarm, but do not explain explicitly our settings and the differnce between them.}

However, we note that when forwarding peers perform settlements, it may happen that they spend more tokens than they receive, resulting in \textit{negative income}.
Such negative income is due to bottlenecks in the network, where a peer may give more free bandwidth to others than it receives. 
In Appendix~\ref{app:paymodelimpact} we provide measurements on effective download rates gateways can achieve when forwarding peers do not perform settlements.
We also show that both our adaptive threshold and especially a more balanced network can reduce the occurrence of \textit{negative income}.
\gi{Does negative income happen in our model only or in Swarm too? Is it contingent on the choice of settings explained above? Next paragraphs suggest that this can happen in both, but then this should be explicitly explained already here.}

It is challenging to prevent threshold rejections and ensure that paying gateways can always receive their chunks while also preventing peers from being discouraged from sharing their bandwidth through negative income.
We believe that this problem can be solved by more complex policies when forwarders should settle debt but leave the details for future work.

\lj{Come back here.}
We note that in our model, as well as Swarm, peers are free to reject requests that do not give income.
However, neighbors will not transfer tokens before they reach the threshold and also the \reefreshrate has been applied.
% peers have to obey the threshold and \refreshrate, and serve some requests for free before they will receive settlements from their neighbors.
If peers could instead signal a threshold rejection and request neighbors to perform token transfers, this mechanism would allow peers to avoid adhering to the free bandwidth by always signaling a threshold rejection.


==> tex/plots/incomeFairenessNew.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
            \input{tex/plots/income-100.tex}
        }
    \caption{\incomefairness for $100\%$ gateways, each requesting $10$ chunks per second.}
    \label{subfig:income-fairness-refresh-100gateway}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
            \input{tex/plots/income.tex}
        }
    \caption{\incomefairness for $0.5\%$ gateways, each requesting $2,000$ chunks per second.\vhl{this can be a bar plot.}}
    \label{subfig:ncome-fairness-refresh-05gateway}
    \end{subfigure}
    \caption{\textit{Limited free service and \incomefairness} 
The effect of limited free service on \incomefairness with $0.5\%$ and $100\%$ gateways. Fairness measurements are included without free service (No free S.), where the \refreshrate is set to zero, with Adjustable free service (Adj. free S.) with an adjustable threshold and \refreshrate, with free service (free S.) with a constant threshold and \refreshrate, and considering only the accounting layer (Acc. only).}
    \label{fig:incomefairnessrefresh}
\end{figure*}

==> tex/plots/paypercentmatrix.tex <==
\begin{figure*}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            % Preamble: \pgfplotsset{width=7cm,compat=1.18}
        \pgfplotsset{height=4cm,width=6.5cm}
        \begin{tikzpicture}
        \begin{axis}[enlargelimits=false,
            % ylabel={secs with $50\times200$ rps},
            colorbar horizontal,
            colorbar style={
                at={(0.5,1.03)},
                anchor=south,
                xticklabel pos=upper,
            },
            xlabel={hops},
            ylabel={seconds},
            point meta min=0,
            point meta max=1,
            symbolic y coords={10,20,30},
            ytick={10,20,30},
            xtick={1,2,3,4,5,6},
            colormap={reverse}{color(0)=(red) color(0.5)=(yellow) color(1)=(green!70!gray)}]
            \addplot [
                matrix plot,
                nodes near coords,
                node near coords style={yshift=-0.25cm},
                % mesh/cols=3,
                point meta=explicit,
            ] table [meta expr=\thisrow{C}, col sep=comma] {data/hoppayedpercentnorecO05.csv};
        \end{axis}
        \end{tikzpicture}    
        }
        \caption{Fraction of paid forwarded chunks with $\mp=16$ and no reciprocity, using a fixed free service on each threshold and direction. $0.5\%$ gateways each requesting $2,000$ chunks per second.}
        \label{subfig:payfractionhonNorec}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
        \pgfplotsset{height=4.5cm,width=6.5cm}
        \begin{tikzpicture}
            \begin{axis}[enlargelimits=false,
                % colorbar,
                ylabel={seconds},
                xlabel={hops},
                point meta min=0,
                point meta max=1,
                symbolic y coords={10,20,100,1000},
                ytick={10,20,100,1000},
                xtick={1,2,3,4,5,6},
                colormap={reverse}{color(0)=(red) color(0.5)=(yellow) color(1)=(green!70!gray)}]
                \addplot [
                    matrix plot,
                    nodes near coords,
                    node near coords style={yshift=-0.25cm},
                    % mesh/cols=3,  
                    point meta=explicit,
                ] table [meta expr=\thisrow{C}, col sep=comma] {data/hoppayedpercentreciprocityO05.csv};
            \end{axis}
            \end{tikzpicture}    
        }
        \caption{Fraction of paid forwarded chunks with $\mp=16$ with reciprocity, allowing to exchange bandwidth for bandwidth.
        $0.5\%$ gateways each requesting $2,000$ chunks per second.}
    \label{subfig:payfractionhonRec}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
            % \input{tex/plots/incomeO05NoRf.tex}
            \input{tex/plots/incomeO05NoRfBar.tex}
        }
        \caption{\incomefairness with $0.5\%$ gateways, with and without reciprocity.}
        \label{subfig:incomeFairnessReciprocityO05}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
        \pgfplotsset{height=4.5cm,width=6.5cm}
        \begin{tikzpicture}
            \begin{axis}[enlargelimits=false,
                % colorbar,
                ylabel={seconds},
                xlabel={hops},
                point meta min=0,
                point meta max=1,
                symbolic y coords={5,10,20},
                ytick={5,10,20},
                xtick={1,2,3,4,5,6},
                colormap={reverse}{color(0)=(red) color(0.5)=(yellow) color(1)=(green!70!gray)}]
                \addplot [
                    matrix plot,
                    nodes near coords,
                    node near coords style={
                        yshift=-0.25cm,
                        /pgf/number format/fixed,
                        /pgf/number format/precision=2,
                    },
                    % mesh/cols=3,
                    point meta=explicit,
                ] table [meta expr=\thisrow{C}, col sep=comma] {data/hoppayedpercentnorecO100.csv};
            \end{axis}
            \end{tikzpicture}    
        }
        \caption{Fraction of paid forwarded chunks with $\mp=16$ and no reciprocity, using a fixed free service on each threshold and direction.
        $100\%$ gateways each requesting $10$ chunks per second.}
    \label{subfig:payfractionhonNoRecAllO}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
        \pgfplotsset{height=4.5cm,width=6.5cm}
        \begin{tikzpicture}
            \begin{axis}[enlargelimits=false,
                % colorbar,
                ylabel={seconds},
                xlabel={hops},
                point meta min=0,
                point meta max=1,
                symbolic y coords={5,100,1000},
                ytick={5,100,1000},
                xtick={1,2,3,4,5,6},
                colormap={reverse}{color(0)=(red) color(0.5)=(yellow) color(1)=(green!70!gray)}]
                \addplot [
                    matrix plot,
                    nodes near coords,
                    node near coords style={
                        yshift=-0.25cm,
                        /pgf/number format/fixed,
                        /pgf/number format/precision=2,
                    },
                    % mesh/cols=3,
                    point meta=explicit,
                ] table [meta expr=\thisrow{C}, col sep=comma] {data/hoppayedpercentreciprocityO100.csv};
            \end{axis}
            \end{tikzpicture}    
        }
        \caption{Fraction of paid forwarded chunks with $\mp=16$ with reciprocity, allowing to exchange bandwidth for bandwidth.
        $100\%$ gateways each requesting $10$ chunks per second.}
    \label{subfig:payfractionhonRecAllO}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
            \input{tex/plots/incomeO100NoRf.tex}
        }
        \caption{\incomefairness with $100\%$ gateways, with and without reciprocity.}
        \label{subfig:incomeFairnessReciprocityO100}
    \end{subfigure}
    \caption{\textit{Reciprocity and \incomefairness} The effect of reciprocity on \incomefairness with $0.5\%$ and $100\%$ gateways.
    Fairness measurements are included with reciprocity (Recip.), without reciprocity (No recip.) and considering only the accounting layer (Acc. only).}
    \label{fig:reciprocity}
\end{figure*}

==> tex/plots/paypercentmatrix100.tex <==
\begin{figure*}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
        \pgfplotsset{height=4.5cm,width=6.5cm}
        \begin{tikzpicture}
            \begin{axis}[enlargelimits=false,
                % colorbar,
                ylabel={seconds},
                xlabel={hops},
                point meta min=0,
                point meta max=1,
                symbolic y coords={5,10,20},
                ytick={5,10,20},
                xtick={1,2,3,4,5,6},
                colormap={reverse}{color(0)=(red) color(0.5)=(yellow) color(1)=(green!70!gray)}]
                \addplot [
                    matrix plot,
                    nodes near coords,
                    node near coords style={
                        yshift=-0.25cm,
                        /pgf/number format/fixed,
                        /pgf/number format/precision=2,
                    },
                    % mesh/cols=3,
                    point meta=explicit,
                ] table [meta expr=\thisrow{C}, col sep=comma] {data/hoppayedpercentnorecO100.csv};
            \end{axis}
            \end{tikzpicture}    
        }
        \caption{Fraction of paid forwarded chunks with $\mp=16$ and no reciprocity, using a fixed free service on each threshold and direction.
        $100\%$ gateways each requesting $10$ chunks per second.}
    \label{subfig:payfractionhonNoRecAllO}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
        \pgfplotsset{height=4.5cm,width=6.5cm}
        \begin{tikzpicture}
            \begin{axis}[enlargelimits=false,
                % colorbar,
                ylabel={seconds},
                xlabel={hops},
                point meta min=0,
                point meta max=1,
                symbolic y coords={5,100,1000},
                ytick={5,100,1000},
                xtick={1,2,3,4,5,6},
                colormap={reverse}{color(0)=(red) color(0.5)=(yellow) color(1)=(green!70!gray)}]
                \addplot [
                    matrix plot,
                    nodes near coords,
                    node near coords style={
                        yshift=-0.25cm,
                        /pgf/number format/fixed,
                        /pgf/number format/precision=2,
                    },
                    % mesh/cols=3,
                    point meta=explicit,
                ] table [meta expr=\thisrow{C}, col sep=comma] {data/hoppayedpercentreciprocityO100.csv};
            \end{axis}
            \end{tikzpicture}    
        }
        \caption{Fraction of paid forwarded chunks with $\mp=16$ with reciprocity, allowing to exchange bandwidth for bandwidth.
        $100\%$ gateways each requesting $10$ chunks per second.}
    \label{subfig:payfractionhonRecAllO}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
            \input{tex/plots/incomeO100NoRf.tex}
        }
        \caption{\incomefairness with $100\%$ gateways, with and without reciprocity.}
        \label{subfig:incomeFairnessReciprocityO100}
    \end{subfigure}
    \caption{\textit{Reciprocity and \incomefairness} with 100\% gateways. The effect of reciprocity on \incomefairness with $100\%$ gateways.
    Fairness measurements are included with reciprocity (Recip.), without reciprocity (No recip.) and considering only the accounting layer (Acc. only).}
    \label{fig:reciprocity}
\end{figure*}

==> tex/plots/varying_workload_cache_accounting.tex <==
\begin{figure*}[t]
    % \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
            \input{tex/plots/varying_workload_incomefairness_cache_accounting.tex}
        }
        \caption{\textit{\incomefairness} for the accounting layer experiment with cache enabled.}
        \label{subfig:incomeFairnessCache}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%     
        \input{tex/plots/varying_workload_incomefairness_cache_accounting_hitratio.tex}
        }
        \caption{Cache hit ratio at all nodes level and Gateways level}
        \label{subfig:cacheHitRatio}
    \end{subfigure}
    \caption{Increasing the load makes the \incomefairness worse.}
    \label{fig:acconting_varyingworkload_cache}
\end{figure*}

==> tex/wip_gateway.tex <==
\section{WIP - Gateway}
A gateway in a decentralized p2p storage network serves as an interface that connects the decentralized network to the outside world, including clients, applications, and other networks. The primary function of a gateway is to enable seamless data exchange and access, abstracting the complexities of the underlying decentralized infrastructure. Several key aspects define the role and significance of a gateway within such networks: 
\begin{itemize}
    \item Data Access and Retrieval: One of the primary functions of a gateway is to provide a means for users or applications to access and retrieve data stored within the decentralized network. It serves as a bridge between the decentralized storage layer and external requests. 
    \item Routing and Discovery: Gateways assist in routing requests to the appropriate peers within the decentralized network. They utilize various discovery mechanisms to locate the peers holding the requested data or to identify suitable peers for storing new data. 
    \item Protocol Translation: Decentralized p2p storage networks may employ specific communication protocols and data formats. Gateways can perform protocol translation when necessary to ensure compatibility with external systems or standards. 
    \item Load Balancing: Gateways can implement load-balancing strategies to evenly distribute incoming requests among available peers. This helps optimize network performance and resource utilization. 
    \item Redundancy and Reliability: To enhance the reliability of data access, gateways may maintain redundant copies of critical data or have failover mechanisms in place. This minimized disruptions in case of peer failures. 
    \item Caching: Gateways can incorporate caching mechanisms to improve data retrieval speed. Frequently accessed data can be temporarily stored at the gateway, reducing the need to retrieve it from the decentralized network repeatedly. 
    \item Metrics and Monitoring: Gateways often provide metrics and monitoring capabilities, allowing network administrators or users to track the performance and health of the network. The collected data can be valuable for optimizing network operations. 
\end{itemize}

While gateways in decentralized p2p storage networks serve important functions, they can indeed introduce certain challenges and potential threats to decentralization. It's crucial to carefully manage these aspects to maintain the core principles of decentralization. Here is a list of challenges and threats to decentralization posed by gateways:
\begin{itemize}
    \item Centralization of Control: One of the primary concerns with gateways is the potential for centralization of control. If a small number of gateways dominate the network, they can exert significant influence over data access, security, and routing. This centralization undermines the core principle of decentralization, where power and control should be distributed among network participants. 
    \item Single Point of Failure: Gateways can become the single point of failure in a decentralized network. If a gateway experiences downtime or is compromised, it can disrupt the entire network's ability to function properly. This vulnerability contradicts the resilience and fault tolerance typically associated with decentralized architectures.
    \item Privacy and Security Risks: Gateways may introduce privacy and security risks, especially if they handle sensitive data or authentication processes. A compromised gateway can lead to unauthorized access, data breaches, and privacy violations. This compromises the security advantages of decentralization.
    \item Governance and Trust Issues: Gateways often require some level of governance and trust. Decisions about which nodes to route requests to, and how data is stored and accessed may involve centralized decision-making. This can erode the trustless nature of decentralized networks.
    \item Economic Incentives: Gateways may introduce economic incentives that encourage centralization. For example, if running a gateway becomes highly profitable, it may attract a concentration of resources and nodes around a few gateways, leading to economic centralization within the network. 
    \item Regulatory Pressure: Gateways may become targets of regulatory authorities seeking to impose control or surveillance on decentralized networks. This can lead to legal and compliance challenges that could compromise the network's decentralized nature. 
\end{itemize}

Taking into consideration the various aspects of a gateway, this paper explores the potential utilization of available free bandwidth by a gateway.

In the bee code (the Swarm client) specific parameters are defined. These parameters include a payment threshold of $100,000,000$ accounting units, a refresh rate of $4,500,000$ accounting units, and a base price of $10,000$ accounting units for each chunk. Notably, the Bee code employs $32$ bytes for addressing both nodes and chunks. However, the formula used to calculate the distance yields values within the range of $1$ to $31$, effectively capping it at $31$ for values exceeding this limit. Consequently, the minimum required accounting units to download a chunk amount to $10,000$, while the maximum stands at $310,000$. By dividing the payment threshold by the maximum required accounting units, we can determine the maximum number of free chunks that can be downloaded per connection under the worst-case scenario which is $322$. Furthermore, dividing the refresh rate by the most expensive chunks results in $15$ chunks.

\vhpl{Continue here.}

==> tex/wip_scope.tex <==

%For the intro?
The nodes in DSS systems experience uneven request loads.
These imbalances may stem from content popularity, uneven node distribution, as well as different connectivity and functionality.
Previous work has studied different mechanisms to reduce such imbalances. 

In this work, we focus on the effect such an imbalanced load has on the distribution of rewards. 
We show that distribution of reward tokens can be even more unbalanced than load distribution. However, careful initialization can also cause reward tokens to be spread more even, than the request load, or can even incentivize more even spread of requests.
\veg{what is initialization? Need to explain before when you explain the problem}

%For the model:
Peers may experience imbalanced load, where some peers receive more requests than others.
Previous work has investigated how load can be spread to multiple peers.

In this work we mainly aim to study how such imbalanced load affects peers income.
While imbalanced load will typically result in imbalanced income, different accounting mechanisms can cause income to be more, or less balanced than the underlying load.
Additionally, we also investigate the effect, accounting mechanisms have on the load distribution, possibly favoring a more even distribution of load.

